End-to-End Keyword Spotting on FPGA Using Graph Neural Networks with a Neuromorphic Auditory Sensor

With the rapid growth of mobile robotics and embedded intelligence, there is an increasing demand for efficient on-device data processing on edge platforms. A promising research direction is the use of neuromorphic sensors inspired by human sensory systems, which generate sparse, event-based data encoding changes in the environment. In this work, we present the first end-to-end FPGA implementation of a keyword spotting system that integrates a Neuromorphic Auditory Sensor (NAS) and a graph neural network (GNN) on a single FPGA device, enabling real-time processing of raw audio data. The proposed architecture eliminates conventional signal preprocessing and operates directly on event-based audio streams. Leveraging a compute-near-memory network architecture, the system achieves efficient inference with low latency and low power consumption. Experimental results demonstrate an accuracy of 87.43% after quantization on the Google Speech Commands v2 dataset processed through the neuromorphic sensor, with end-to-end latency below 35 us and average power consumption of 1.12 W. The processed datasets, software models, and hardware modules are available at https://github.com/vision-agh/NAS-GNN-KWS.

==> figures/statistics/table_plots.tex <==
\begin{table}[!ht]
\centering
\caption{Statistics of the generated neuromorphic version of the Google Speech Commands v2 dataset.}
\label{tab:statistics}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Version} &
\textbf{Max. ev./sample} &
\textbf{Avg. ev./sample} &
\textbf{Max. ev./s} &
\textbf{Avg. ev./s} &
\textbf{Max. ev./10 ms} &
\textbf{Avg. ev./10 ms} \\
\midrule
32-serial    & 204839 & $17217 \pm 9576$   & 151209 & $15025 \pm 8215$   & 2811 & $150 \pm 209$ \\
32-paraller  &        &                   &        &                   &      &               \\
64-serial    & 227995 & $31673 \pm 13963$  & 194637 & $31673 \pm 13963$  & 3990 & $244 \pm 301$ \\
64-paraller  & 245346 & $75404 \pm 21410$  & 277070 & $54013 \pm 16142$  & 7893 & $536 \pm 506$ \\
128-serial   & 254669 & $61266 \pm 20943$  & 240573 & $45488 \pm 16010$  & 5477 & $452 \pm 474$ \\
128-paraller &        &                   &        &                   &      &               \\
\bottomrule
\end{tabular}%
}
\end{table}





\pgfplotstableread[col sep=comma]{figures/statistics/events_per_channel_stats_32_serial.csv}\TserialA
% \pgfplotstableread[col sep=comma]{figures/statistics/events_per_channel_stats_32_parallel.csv}\TparA

\pgfplotstableread[col sep=comma]{figures/statistics/events_per_channel_stats_64_serial.csv}\TserialB
\pgfplotstableread[col sep=comma]{figures/statistics/events_per_channel_stats_64_parallel.csv}\TparB

\pgfplotstableread[col sep=comma]{figures/statistics/events_per_channel_stats_128_serial.csv}\TserialC
% \pgfplotstableread[col sep=comma]{figures/statistics/events_per_channel_stats_128_parallel.csv}\TparC

\begin{figure}[t]
\centering
\begin{tikzpicture}

% --- Define colors once (pick whatever you like) ---
\definecolor{SerialCol}{RGB}{0,114,178}   % blue-ish
\definecolor{ParCol}{RGB}{213,94,0}       % orange-ish

\begin{groupplot}[
    group style={
        group size=1 by 3,
        vertical sep=3.8ex,
        x descriptions at=edge bottom,
        y descriptions at=edge left,
        xticklabels at=all,
    },
    width=\columnwidth,
    height=0.33\columnwidth,
    grid=both,
    tick align=outside,
    tick pos=left,
    ymin=0,
    xlabel={Channel index},
    ylabel={Avg. \#events},
    label style={font=\small},
    ticklabel style={font=\small},
    x tick label style={/pgf/number format/fixed, yshift=1pt},
    xticklabel style={font=\small},
    title style={font=\small},
    legend style={
        draw=none,
        fill=none,
        font=\small,
        at={(0.02,0.98)},
        anchor=north west
    },
]

% ---------------- Panel 1: 32 ----------------
\nextgroupplot[
    xtick={0,16,32,48,64},
]

\node[anchor=north east, font=\small\bfseries] at (axis description cs:0.98,0.98) {(a) 32 ch};

% mean (serial)
\addplot[thick, mark=none, color=SerialCol, name path=meanS32]
    table[x=channel, y=mean] {\TserialA};
\addlegendentry{serial}

% upper/lower (serial)
\addplot[draw=none, name path=upperS32]
    table[x=channel, y expr=\thisrow{mean}+\thisrow{std}] {\TserialA};
\addplot[draw=none, name path=lowerS32]
    table[x=channel, y expr=\thisrow{mean}-\thisrow{std}] {\TserialA};

% fill band (serial)
\addplot[fill=SerialCol, fill opacity=0.18, draw=none]
    fill between[of=upperS32 and lowerS32];

% % parallel (keep commented if you want)
% \addplot[thick, dashed, mark=none, color=ParCol, name path=meanP32]
%     table[x=channel, y=mean] {\TparA};
% \addlegendentry{parallel}
%
% \addplot[draw=none, name path=upperP32]
%     table[x=channel, y expr=\thisrow{mean}+\thisrow{std}] {\TparA};
% \addplot[draw=none, name path=lowerP32]
%     table[x=channel, y expr=\thisrow{mean}-\thisrow{std}] {\TparA};
% \addplot[fill=ParCol, fill opacity=0.12, draw=none]
%     fill between[of=upperP32 and lowerP32];

% ---------------- Panel 2: 64 ----------------
\nextgroupplot[
    xtick={0,32,64,96,128},
]
\node[anchor=north east, font=\small\bfseries] at (axis description cs:0.98,0.98) {(b) 64 ch};
% mean (serial)
\addplot[thick, mark=none, color=SerialCol, name path=meanS64]
    table[x=channel, y=mean] {\TserialB};

% upper/lower (serial)
\addplot[draw=none, name path=upperS64]
    table[x=channel, y expr=\thisrow{mean}+\thisrow{std}] {\TserialB};
\addplot[draw=none, name path=lowerS64]
    table[x=channel, y expr=\thisrow{mean}-\thisrow{std}] {\TserialB};

% fill band (serial)
\addplot[fill=SerialCol, fill opacity=0.18, draw=none]
    fill between[of=upperS64 and lowerS64];

% mean (parallel)
\addplot[thick, dashed, mark=none, color=ParCol, name path=meanP64]
    table[x=channel, y=mean] {\TparB};

% upper/lower (parallel)
\addplot[draw=none, name path=upperP64]
    table[x=channel, y expr=\thisrow{mean}+\thisrow{std}] {\TparB};
\addplot[draw=none, name path=lowerP64]
    table[x=channel, y expr=\thisrow{mean}-\thisrow{std}] {\TparB};

% fill band (parallel)
\addplot[fill=ParCol, fill opacity=0.12, draw=none]
    fill between[of=upperP64 and lowerP64];

% ---------------- Panel 3: 128 ----------------
\nextgroupplot[
    xtick={0,64,128,194,256},
]

\node[anchor=north east, font=\small\bfseries] at (axis description cs:0.98,0.98) {(c) 128 ch};

% mean (serial)
\addplot[thick, mark=none, color=SerialCol, name path=meanS128]
    table[x=channel, y=mean] {\TserialC};

% upper/lower (serial)
\addplot[draw=none, name path=upperS128]
    table[x=channel, y expr=\thisrow{mean}+\thisrow{std}] {\TserialC};
\addplot[draw=none, name path=lowerS128]
    table[x=channel, y expr=\thisrow{mean}-\thisrow{std}] {\TserialC};

% fill band (serial)
\addplot[fill=SerialCol, fill opacity=0.18, draw=none]
    fill between[of=upperS128 and lowerS128];

% % parallel (keep commented if you want)
% \addplot[thick, dashed, mark=none, color=ParCol, name path=meanP128]
%     table[x=channel, y=mean] {\TparC};
%
% \addplot[draw=none, name path=upperP128]
%     table[x=channel, y expr=\thisrow{mean}+\thisrow{std}] {\TparC};
% \addplot[draw=none, name path=lowerP128]
%     table[x=channel, y expr=\thisrow{mean}-\thisrow{std}] {\TparC};
% \addplot[fill=ParCol, fill opacity=0.12, draw=none]
%     fill between[of=upperP128 and lowerP128];

\end{groupplot}

\end{tikzpicture}
\caption{Average events per channel with colored mean curves and transparent $\pm 1\sigma$ bands.}
\end{figure}
